Automated, Unsupervised, and Auto-parameterized Inference of Data Patterns and Anomaly Detection

With the advent of data-centric and machine learning (ML) systems, data quality is playing an increasingly critical role in ensuring the overall quality of software systems. Data preparation, an essential step towards high data quality, is known to be a highly effort-intensive process. Although prior studies have dealt with one of the most impacting issues, data pattern violations, these studies usually require data-specific configurations (i.e., parameterized) or use carefully curated data as learning examples (i.e., supervised), relying on domain knowledge and deep understanding of the data, or demanding significant manual effort. In this paper, we introduce RIOLU: Regex Inferencer auto-parameterized Learning with Uncleaned data. RIOLU is fully automated, automatically parameterized, and does not need labeled samples. RIOLU can generate precise patterns from datasets in various domains, with a high F1 score of 97.2%, exceeding the state-of-the-art baseline. In addition, according to our experiment on five datasets with anomalies, RIOLU can automatically estimate a data column's error rate, draw normal patterns, and predict anomalies from unlabeled data with higher performance (up to 800.4% improvement in terms of F1) than the state-of-the-art baseline, even outperforming ChatGPT in terms of both accuracy (12.3% higher F1) and efficiency (10% less inference time). A variant of RIOLU, with user guidance, can further boost its precision, with up to 37.4% improvement in terms of F1. Our evaluation in an industrial setting further demonstrates the practical benefits of RIOLU.

==> sections/5_implementation.tex <==
\section{Pattern Generation implementation}
\label{sec:pattern_generator_implementation}
In this section, we are to introduce the pattern generation\todo{Better call it constraint inference: pattern generation is a broader term} implementation logic of RIOLU. The pattern generator is to solve the CSP\todo{CSP is about constraint selection, whereas this section is about constraint inference?}. A $r_{cov}$ is estimated in either semi-supervised or unsupervised way, as addressed in Sec~\ref{sec:coverage_rate_estimation}. Samples are initially decomposed into templates with \textbf{TOKEN}s and \textbf{delimeter}s according to $r_{cov}$ %\heng{is this the coverage threshold? it should be explained} 
and being clustered according to the templates. %\heng{patterns are clustered, not samples, right?}. 
Each token in a template cluster is then elaborated with the four layers\todo{the layers are used previously when describing CSP but defined here} of constraints (i.e., token range, token length, static characters, static type). Fig~\ref{fig:generation_example} provides an example of the workflow for token constraint generation using five date time records in a template cluster. 

%\heng{I strongly suggest using a running example for the subsections in this section. Create a small dataset (a column) with a small number (e.g., 10) of samples. In each step, explain the action of the step on the small data. Use the same example for all the steps. The details of the steps are explained using the example. Otherwise, it is very challenging to understand the details. An example can be found in this paper: https://www.hengli.org/pdf/Dai2020Logram.pdf: Section 4 with Figures 2 and 3.}

\begin{comment}
    
\subsection{Data Sampling}
%\heng{First explain the purposes of splitting: the purposes of training and testing data}
We sample a subset of data without replacement to learn the patterns \heng{mind the confusion between templates vs patterns: use consistent wording} and calculate their coverage on the whole dataset as their generalizability. The size $N_{tr}$ samples is calculated automatically using a z-score with a confidence level of 95\% and an error margin of 5\%. 

To learn patterns unbiasedly, the training data shall represent the distribution of the corresponding domain.  %\heng{learn X in an unbiased way?}. 
However, given that the dataset is fully unlabeled, the data distribution remains unknown. To represent the dataset in a non-parametrical %\heng{non-parametrical?} 
way, we select the training samples with the bootstrapping method~\cite{efron1992bootstrap}. \heng{To discus the bootstrapping method used. Show the sample size in a table, can be together with the dataset able, referring to the table here.} 


\subsection{Learning Strategy}
\label{sec:learning_strategy}
A set of patterns that satisfy both $\theta_{cov}$ and $\theta_{gain}$ can be selected through a problem-solving process defined in sec~\ref{sec:csp_pattern_generation} and sec~\ref{sec:csp_pattern_selection}. However, given that the dataset is fully unlabeled, drawing samples from the dataset for one loop could result in a biased pattern set. ({\it e.g., }The patterns learned from the current split are scattered, and all have low gains. The trend could cause the cut according to $\theta_{gain}$ being random. ) To fully leverage the knowledge in the dataset, we implement a multiple-loop learning strategy inspired by cross-validation~\cite{mosteller1968data}. 

By each loop, $N_{tr}$ samples from the dataset are drawn with the bootstrapping method~\cite{efron1992bootstrap} as the training set; the unselected samples serve as the testing set. By executing the constraint generation step in each loop, a set of patterns with their $Cov_{tr}(p)$ and $Imp_{te}(p)$ is collected. After collecting all the patterns through $t$ times, they are ranked and filtered according to the average gain. For the $i^{th}$ loop, the gain for each pattern is calculated as: 

\begin{equation}
    Gain_i(p) = 
    \begin{cases}
    \frac{Cov_{tr_i}(p)}{Imp_{te_i}(p)},& \text{if } Cov_{tr_i}\neq 0\\
    0,              & \text{otherwise}
    \end{cases}
\end{equation}

According to the single-loop gains, one can calculate the average gain for each pattern:
\begin{equation}
    \label{eqn:average_gain}
    AvgGain(p) = \frac{1}{t}\sum_{i=1}^t Gain_i(p)
\end{equation}

To construct a variable set for the multiple-loop learning CSP, average gains are then to be or from high to low (i.e., $i<j$ if $AvgGain(p_i)>AvgGain(p_j)$); we shall re-state the CSP for pattern selection as:

\begin{boxD}
$\mathcal{X}_{multi-sel}=\{AvgGain(p_1), ..., AvgGain(p_m)\}$\\
$\mathcal{D}_{multi-sel}=\{\{0, 1\}, \{0, 1\}, ..., \{0, 1\}\}$\\
\begin{math}
\mathcal{C}_{multi-sel}=\biggl\{
    \begin{array}{l}
        \sum_{i=1}^kAvgGain(p_i) >= \theta_{gain},\ if\ k>0\\
        \sum_{i=1}^{k-1}AvgGain(p_i) < \theta_{gain} < \theta_{cov},\ if\ k>0
    \end{array}
\end{math}
\end{boxD}

Based on the variables composed by ranked average gains, multiple loop selection aims to find the minimum positive index $k$ that satisfies the constraints. The first $k^{th}$ patterns will be kept in the final pattern pool. 
\end{comment}



\begin{comment}
\begin{enumerate}
    \item Token range selection
    \item Token length determination
    \item Static character determination
    \item Character type determination
\end{enumerate}


\begin{figure*}[!h]
  \centering
  \includegraphics[width=\textwidth]{images/pattern_generation.pdf}
  \caption{The workflow of constraint generation for a sample token in one template. }
  \label{fig:pattern_generation}
\end{figure*}
\end{comment}



\subsection{Token Length Determination}
\label{sec:token_length_determination}
While a specific content range may not be applicable for a token, there may be a limitation to the length in the corresponding field. %\heng{For such examples (longer than a few words), it's better to start a new sentence with ``For example,'' with out parentheses}
A static length $len$ for a token is determined if and only if most token contents have a fixed length; if the system fails to detect a static length for the current token, a minimum description length will be captured as $len_{Min}$. In our running example Fig~\ref{fig:generation_example}, $TOKEN_1$, $TOKEN_2$, and $TOKEN_3$ have token length constraints for each. 

\subsection{Static Character Determination}
\label{sec:static_character_determination}
For the $i^{th}$ sample in cluster $C$, its $j^{th}$ token $C_{ij}$ could be decomposed into having $m$ character slots and being expressed as $C_{ij1}, ..., C_{ijm}$. We implement a similar strategy with token range selection by using K-Means clustering based on frequencies. The frequencies are calculated through counting the existence time\todo{frequency} for a character on a certain slot (e.g., for the first character slot in $TOKEN_3$, the frequency of ``0'' is 0.2 while the frequency for ``1'' is 0.8). We also insert 1 and $\frac{1}{N_{tr}}$ into the frequency list to ensure the split. For the $k^{th}$ character slot in the $j^th$ token, $C_{1jk}, ..., C_{njk}$ is collected through iterating every sample in the cluster. The static character may branch into two paths according to whether the token has a static length. If a static token length $len$ is detected, the system will stop detecting static character ranges based on the majority of the samples when $k>len$. Otherwise, a static character range will be detected only for the $k^{th}$ slot when $k<=len_{Min}$. \todo{might be better to mention this earlier: what if the length is static, what if not.}

The intuition of the determination border is that, for static length strings, we shall not expect more characters, which could cause a conflict with the length constraint. Conversely, for tokens without length constraints, the part out of the minimum length is too scattered to support a precise character range conclusion. Hence, in this case, static character constraints are only detected for the string slice from the $1^{st}$ slot to the $len_{Min}^{th}$ slot. 

We decompose $TOKEN_3$ in Fig~\ref{fig:generation_example}. The constant length constraint is 5 for this token, and each slot in the token contains five characters as a character pool. For the third slot, the static letter is ``T'', and we determine ``0'' as the static character for the last two slots. However, for the first two slots, no static character is detected. 

\subsection{Static Type Determination}
\label{sec:static_type_determination}
For the $k^{th}$ character slot in the $j^{th}$ token, static type is to be detected if and only if when a range of static characters (i.e., a stricter constraint) fails to be determined; if all types of components (i.e., letters, digits, and symbols) are being detected in the majority of current character slot, the slot would have no constraint and accepts all types of component. The character types are assigned according to the majority types of characters in the current slot. 

Following the intuition in static character determination, the static type constraint only applies when $k<=len$ with a length constraint and $k<=len_{Min}$ without a length constraint. Additionally, if the length constraint does not apply to the token, type suggestions for slot $k$ when $k>len_{Min}$ will be loosened with a $*$, indicating the probability of having all types of candidates. 

Since the first two slots in $TOKEN_3$ do not have static characters, we are to check their static character type. Both slots have a static type of digits, written as ``\textbackslash d''.

\heng{Add a short description: after the determination of the four types, how the pattern is generated.}


==> tables/api_key_categories.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{API key labels and their corresponding verification messages.}
\label{tab:api_key_categories}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Label}   & \textbf{Generated\_by\_OpenAI}                                                                                                    & \textbf{Unknown}                                                                      \\ \hline
\textbf{Message} & \begin{tabular}[c]{@{}c@{}}access\_terminated, account\_deactivated,\\ billing\_not\_active, insufficient\_quota,yes\end{tabular} & \begin{tabular}[c]{@{}c@{}}invalid\_api\_key, empty, \\ no\_organization\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/configurable_parameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[h]
\centering
\caption{The configurable parameters in HiCoPAD, along with their symbol and descriptions.}
\label{tab:configurable_parameters}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{3.5cm}|p{1cm}|p{9cm}@{}}
\hline
\textbf{Parameter}          & \textbf{Symbol} & \textbf{Descriptions}                                                                          \\ \hline
\textbf{Granularity}        &$Gran$& The granularity controls the portion of training samples that delimiters can finely split.     \\ \hline
\textbf{Categorical Threshold} &$\theta_{cat}$&
  The categorical threshold aids the system in determining the maximum number of acceptable bins. \\\hline
\textbf{Coverage Threshold} &$\theta_{cov}$& The coverage threshold represents the majority of the training set in determining constraints. \\\hline
\textbf{Gain Threshold}     &$\theta_{gain}$& The gain threshold serves as a cut in selecting high gain patterns.                 \\\hline
\textbf{Bootstrap Size}     &$N_{tr}$& The number of times executing random selection for training set creation.                      \\\hline
%\textbf{Number of Loops} &$t$&  Number of learning loops; multiple learning loops can be executed to ensure the selected patterns' stability further. \\ \hline
\end{tabular}%
}
\end{table*}
